Improved Streaming Edge Coloring

Given a graph, an edge coloring assigns colors to edges so that no pairs of adjacent edges share the same color. We are interested in edge coloring algorithms under the W-streaming model. In this model, the algorithm does not have enough memory to hold the entire graph, so the edges of the input graph are read from a data stream one by one in an unknown order, and the algorithm needs to print a valid edge coloring in an output stream. The performance of the algorithm is measured by the amount of space and the number of different colors it uses. This streaming edge coloring problem has been studied by several works in recent years. When the input graph contains $n$ vertices and has maximum vertex degree $\Delta$, it is known that in the W-streaming model, an $O(\Delta^2)$-edge coloring can be computed deterministically with $\tilde{O}(n)$ space [Ansari, Saneian, and Zarrabi-Zadeh, 2022], or an $O(\Delta^{1.5})$-edge coloring can be computed by a $\tilde{O}(n)$-space randomized algorithm [Behnezhad, Saneian, 2024] [Chechik, Mukhtar, Zhang, 2024]. In this paper, we achieve polynomial improvement over previous results. Specifically, we show how to improve the number of colors to $\tilde{O}(\Delta^{4/3+\epsilon})$ using space $\tilde{O}(n)$ deterministically, for any constant $\epsilon > 0$. This is the first deterministic result that bypasses the quadratic bound on the number of colors while using near-linear space.

==> overview.tex <==
\subsection{Technical Overview}
In this part, we give an informal overview of our algorithm. 

\tianyi{We should first give a brief overview of [BS24], and then focus on our typical $(1, \Delta^{1/2})$-case. As an overview, we only need to show how to break $\Delta^{1.5}$ to achieve $\Delta^{1.25}$ on this hard example. After that, we briefly explain other technical difficulties which worsen the bound. I can help to write something like this}

Our intuition here is that instead of processing a group of edges adjacent to an online vertex each time, we consider a batch of $O(n)$ edges consisting of many groups. We use $B_1, B_2, \cdots, B_\Delta$ to denote the $i$-th batch of edges in the order it comes. Each batch consists of some groups, where each group is a star centered at an online vertex of at least $\Delta^{3/7}$ vertices. Suppose we are processing $B_i$, and let $G_i$ denote the edge-induced subgraph of $B_i$. Let $\Delta_i^{\text{online}}$ and $\Delta_i^{\text{offline}}$ denote the maximum degree of online and offline vertices of $G_i$ separately. By the assumption before, we know $\Delta_i^{\text{online}}, \Delta_i^{\text{offline}} \in [\Delta^{3/7}, \Delta^{4/7}]$. 

Next, we discuss two situations：The first case is balanced case, that is, $\forall v \in \text{offline}_i, \deg_i \ge \Delta^{1/7}$. Another case is unbalanced case. That is, $\forall v \in \text{offline}_i, \deg_i \le \Delta^{1/7}$

\paragraph{Balanced case: }
If we use the method in \cite{behnezhad2023}, we need a palette of size $\Delta^{4/7} \times O(\log \Delta) \times \Delta = \Tilde O(\Delta^{11/7})$ here, since there are at most $\Delta / \Delta^{3/7} = \Delta^{4/7}$ groups for each online vertex, and we need a table of size $ [O(\log \Delta)] \times [\Delta]$ for each offline vertex.

Consider an offline vertex $v$. 
%, suppose the edges incident to $v$ are $u_1v, u_2v, u_3v, \cdots$ in the order revealed. 
The color of an edge $uv$ is a triple $(b_u, i, (r_v^i + c_v) \bmod C)$. In the previous coloring, if we fix $x \in [O(\log \Delta)], y \in [\Delta]$, at most one color is used among all colors of form $(\cdot, x, y)$. This is because whenever we reveal an edge, the counter $c_v$ is increased by $1$. However, we can slightly modify the algorithm such that we only increase the counter when we reveal the whole batch of edges instead of an edge. In this way, we will increase the counter at most $\Delta / \Delta^{1/7} = \Delta^{6/7}$ times, thus reducing the palette size to $\Delta^{4/7} \times O(\log \Delta) \times \Delta^{6/7} = O(\Delta^{10/7})$.

But this modification will cause new problems. Suppose edges incident to $v$ in this batch are $u_1v, u_2v, \cdots, u_kv$. The colors of these edges may conflict. This happens when $u_i$ and $u_j$ share the same batch number, i.e. $b_{u_i} = b_{u_j}$. To avoid this, We can assign a random shift $r'_u$ for each online vertex $u$ and $b'_u = (b_u + r'_u) \bmod \Delta^{4/7}$. Instead of color an edge with $(b_u, \cdot, \circ)$, now we use color $\left(b'_u, \cdot, \circ \right)$. In this way, since $\Delta_{i}^{\text{online}} \le \Delta^{4/7}$, at least half of $b'_u$ is unique and we color the corresponding edges with these unique color. Extending it to $O(\log n)$ random shifts as before, we can successfully color all edges.

\paragraph{Unbalanced case: }
We consider a more extreme case where $\forall v \in \text{offline}_i, \deg_i = 1$ here. 

We divide the batches into phases, such that each phase consists of $k = O(\Delta^{1/2})$ batches. Denote the edges set of each phase is $P_1, P_2, \cdots, P_{k}$. Call an online vertex $v$ heavy at phase $i$ if $\deg_{G[P_i]}(v) \ge \Delta^{5/7}$, and light otherwise.

\subparagraph{Light Vertices}
First, we consider how to color the edges in a phase. For light vertices, we know that each group consists of $\Delta^{3/7}$ edges, and total edges in a phase is no more than $\Delta^{5/7}$. Thus each online vertex participate in $O(\Delta^{2/7})$ batches. Combining that degree of offline vertex is at most $1$ in a batch, we need to use a palette of $[\Delta^{2/7}] \times [\Delta^{1/2}]$. 
For different phases, we just need to append the phase number to the current color. Thus in total we use $\Delta^{2/7} \times \Delta^{1/2} \times \Delta^{1/2} = \Delta^{9/7}$ colors. 

\subparagraph{Heavy Vertices}
For any offline vertex $u$, it appears as heavy vertex at most $O(\Delta / \Delta^{5/7} = \Delta^{2/7}$ times. 
Suppose for any phase, we can color it using $\Delta$ colors. By appending the phase number to the current color, we use $\Delta \times \Delta^{2/7} = \Delta^{9/7}$ colors in total.

\subparagraph{From degree $1$ to degree $\Delta^{1/7}$}

Denote the above algorithm for $\Delta_i^{\text{offline}} = 1$ case by $\mathcal A$. Note that if the degree of online vertex is smaller than $\Delta^{3/7}$, $\mathcal A$ still works. We just need to divide the graph $G_i$ into $O(\Delta^{1/7})$ graphs $G'_i$ whose maximum degree in the offline part is $1$. And run $\mathcal A$ for each $G'_i$. For an edge in $G'_i$ of color $c$ returned by $\mathcal A$, we output $(c, i)$. Thus we use $O(\Delta^{9/7} \times \Delta^{1/7}) = O(\Delta^{10/7})$ colors in total.

